OpenVision: A Fully-Open, Cost-Effective Family of Advanced Vision Encoders for Multimodal Learning

OpenAI's CLIP, released in early 2021, have long been the go-to choice of vision encoder for building multimodal foundation models. Although recent alternatives such as SigLIP have begun to challenge this status quo, to our knowledge none are fully open: their training data remains proprietary and/or their training recipes are not released. This paper fills this gap with OpenVision, a fully-open, cost-effective family of vision encoders that match or surpass the performance of OpenAI's CLIP when integrated into multimodal frameworks like LLaVA. OpenVision builds on existing works -- e.g., CLIPS for training framework and Recap-DataComp-1B for training data -- while revealing multiple key insights in enhancing encoder quality and showcasing practical benefits in advancing multimodal models. By releasing vision encoders spanning from 5.9M to 632.1M parameters, OpenVision offers practitioners a flexible trade-off between capacity and efficiency in building multimodal models: larger models deliver enhanced multimodal performance, while smaller versions enable lightweight, edge-ready multimodal deployments.

==> table_openness.tex <==
\small
\begin{tabular}{l|>{\columncolor{green!80!black!15}}c|>{\columncolor{green!80!black!15}}c|>{\columncolor{green!80!black!15}}c|>{\columncolor{green!80!black!15}}c|>{\columncolor{green!80!black!15}}c|>{\columncolor{green!80!black!15}}c|}
\rowcolor{white}
\multicolumn{1}{c}{} & \multicolumn{1}{c}{Data Open} & \multicolumn{1}{c}{Training Code Open} & \multicolumn{1}{c}{Evaluation Open} & \multicolumn{1}{c}{Model Number} & \multicolumn{1}{c}{Training Hours} & \multicolumn{1}{c}{Release Date} \\ \hhline{|~|------|}
OpenAI's CLIP &  {} & {} & \cellcolor{green!80!black!10}{\boldcheckmark} & {$4$} & {04/2025} & {04/2025} \\ \hhline{|~|------|}
Google's SigLIP &  {} & {} & \cellcolor{green!80!black!10}{\boldcheckmark}  & {$10$} & {04/2025} & {04/2025} \\ \hhline{|~|------|}
OpenVision (Ours) &  \cellcolor{green!80!black!10}{\boldcheckmark} & \cellcolor{green!80!black!10}{\boldcheckmark}  & \cellcolor{green!80!black!10}{\boldcheckmark}  & \cellcolor{green!80!black!10}{$\approx 27$} & \cellcolor{green!80!black!10}{04/2025} & {04/2025} \\ \hhline{|~|------|}

\end{tabular}

